Strong broadband intensity noise squeezing from near-infrared to terahertz frequencies in semiconductor lasers with nonlinear dissipation

The generation and application of squeezed light have long been central goals of quantum optics, enabling sensing below the standard quantum limit, optical quantum computing platforms, and more. Intensity noise squeezing of bright (coherent) states, in contrast to squeezed vacuum, is relatively underdeveloped. Bright squeezing has been generated directly through nonlinear optical processes or ``quietly pumped'' semiconductor lasers. However, these methods suffer from weak squeezing limits, narrow operating wavelength ranges, and have not been explored at large bandwidths. Here, we show how semiconductor lasers with sharp intensity-dependent dissipation can support highly broadband intensity noise squeezing from infrared (IR) to terahertz (THz) wavelengths, the latter of which has remained unexplored in quantum noise studies. Our protocol realizes strongly ($>10$ dB) intensity noise-squeezed intracavity quantum states, which could create a new regime for cavity quantum electrodynamics experiments, as well as strong output squeezing surpassing gigahertz bandwidths. Furthermore, we show how the same systems also create self-pulsing and bistable mean field behavior, enabling control of light in both the temporal and noise domains. The existence of these multiple functionalities in both the classical and quantum mechanical domains in a single semiconductor laser platform, from IR to THz wavelengths, could enable advances in on-chip quantum optical communication, computing, and sensing across the electromagnetic spectrum.

==> preamble.tex <==
%-----CHANGING CITATION APPEARANCE----
\setcitestyle{numbers,square,sort&compress} %We don't want the rmp citation style, but standard style square bracket, numbers style instead

%----KERNING-----
\usepackage{microtype} %For better kerning and symbol-stretching
\usepackage{xspace} %For the \xspace command

%----LOADING RELEVANT FONTS [TIMES ROMAN FOR PRB] -----
\usepackage{txfonts}  %Times Roman fonts
\usepackage{txfontsb} %Addition for txfonts, including old style numerals and greek
%					  %\usepackage{mathptmx} Also a Times Roman Font
%\usepackage{bm} %Bold math symbols with \bm{} (Greek and other symbols)
%\usepackage{mnsymbol} %For llangle and rrangle

%-----CROSS-REFERENCING-----
\usepackage{xr}

%-----COLOR AND GRAPHICS PACKAGES-----
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}

%-----SETTINGS FOR REFERENCES-----
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    linkcolor={blue!75!black!80!yellow},
    citecolor={blue!75!black!80!yellow},
    urlcolor={blue!75!black!80!yellow}
}

%-----PACKAGE FOR BOXED MULTI-LINE EQUATIONS-----
\usepackage{empheq}
\newcommand*\widefbox[1]{\fbox{\hspace{2em}#1\hspace{2em}}}

%-----CHANGE MARGINS OF DOCUMENT-----
\usepackage[top=1in, bottom=1.5in, left=1.4in, right=1.4in]{geometry} %Change margins

%-----SOME SETTINGS FOR MARGINPAR-----
%\usepackage{marginfix} %Should fix even more than mparhack, so use this instead unless you see something funky

\let\oldmarginpar\marginpar %This and the next line changes the fontsize
\def\marginpar#1{\oldmarginpar{\scriptsize #1}}
\setlength{\marginparwidth}{6.5em} %Changes the width of the note
\setlength{\marginparsep}{2em} %Probably enforces a minimum distance between marginpar-notes


%INCLUDING CLEVEREF PACKAGE FOR MORE CONVENIENT REFERENCING ABILITIES
\usepackage[capitalize,nameinlink]{cleveref}
\newcommand{\crefrangeconjunction}{\,--\,}
\crefname{subequations}{Eqs.}{Eqs.} %Specific changes to allow for Eqs.-wording when referring to a set of subequations. Label of subequations must include [subequations] as an option.
\Crefname{subequations}{Eqs.}{Eqs.}
\crefformat{subequations}{#2Eqs.~(#1)#3}
\Crefformat{subequations}{#2Eqs.~(#1)#3}
\crefname{page}{p.}{p.} %Changing from 'page' to 'p.'
\newcommand{\heqref}[1]{\hyperref[#1]{(\ref*{#1})}} %Alternative to \eqref, which works better with hyperlinks (whole thing is clickable)
\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable
\newcommand{\namedeqref}[2]{\hyperref[#2]{#1~(\ref*{#2})}} %\nameref{Name}{label} will produce Name~\ref{label} with the entire thing clickable


%-----PACKAGE TO ALLOW CHANGING OF ENUMERATE BULLETS-----
\usepackage{enumitem}

%-----COMMANDS-----
\newcommand{\vek}[1]{\mathbf{#1}}
\newcommand{\rv}{\mathbf{r}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\nablav}{\boldsymbol{\nabla}}
\newcommand{\hxv}{\hat{\mathbf{x}}}
\newcommand{\hyv}{\hat{\mathbf{y}}}
\newcommand{\ef}{\epsilon_{\text{\textsc{f}}}}
\newcommand{\vf}{v_{\text{\textsc{f}}}}
\newcommand{\tsc}[1]{\text{\textsc{#1}}}
\newcommand{\kb}{k_\tsc{b}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddb}[1]{\!\dd#1\,}
\newcommand{\dde}{\,\dd}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern.2pt}\sim\cr\noalign{\kern-2.5pt}}}}}

\newcommand{\spar}{_{\scriptscriptstyle\parallel}}
\newcommand{\kpar}{k_{\scriptscriptstyle\parallel}}
\newcommand{\kvpar}{\kv_{\scriptscriptstyle\parallel}}
\newcommand{\rpar}{r_{\scriptscriptstyle\parallel}}
\newcommand{\rvpar}{\rv_{\scriptscriptstyle\parallel}}
\newcommand{\vpar}{v_{\scriptscriptstyle\parallel}}
\newcommand{\vvpar}{\vv_{\scriptscriptstyle\parallel}}
\newcommand{\dperp}{d_{\perp}}
\newcommand{\dpar}{d_{\parallel}}
\newcommand{\iu}{\mathrm{i}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\sgn}{\operatorname{sgn}}

\newcommand{\pr}[1]{|#1\rangle\langle#1|}
\newcommand{\prsf}[1]{\mathsf{|#1\rangle\langle#1|}}

\newcommand{\Ev}{\mathbf{E}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Hv}{\mathbf{H}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\dv}{\mathbf{d}}
\newcommand{\hv}{\mathbf{h}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\Gv}{\mathbf{G}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\nv}{\hat{\mathbf{n}}}

%abbreviations
\newcommand{\ie}{i.e.\@\xspace} %Gobble-spaces of the "small" type (small is ensured by adding \@)
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
